Compact: Approximating Complex Activation Functions for Secure Computation

Secure multi-party computation (MPC) techniques can be used to provide data privacy when users query deep neural network (DNN) models hosted on a public cloud. State-of-the-art MPC techniques can be directly leveraged for DNN models that use simple activation functions such as ReLU. However, these techniques are ineffective and/or inefficient for the complex and highly non-linear activation functions used in cutting-edge DNN models. We present Compact, which produces piece-wise polynomial approximations of complex AFs to enable their efficient use with state-of-the-art MPC techniques. Compact neither requires nor imposes any restriction on model training and results in near-identical model accuracy. To achieve this, we design Compact with input density awareness and use an application-specific simulated annealing type optimization to generate computationally more efficient approximations of complex AFs. We extensively evaluate Compact on four different machine-learning tasks with DNN architectures that use popular complex AFs silu, gelu, and mish. Our experimental results show that Compact incurs negligible accuracy loss while being 2x-5x computationally more efficient than state-of-the-art approaches for DNN models with large number of hidden layers. Our work accelerates easy adoption of MPC techniques to provide user data privacy even when the queried DNN models consist of a number of hidden layers and trained over complex AFs.

==> figures/approximation_difference.tex <==
\begin{figure}
    \includegraphics[width=\columnwidth]{figures/Differences.png}
    \caption{}
    \label{fig:before-and-after-normalization}
\end{figure}



==> sections/summary-of-changes.tex <==
\onecolumn
% \title*{Summary of Changes}
\newcommand{\ans}[1]{{\color{black}\smallskip\noindent{\bf Response:} #1}} 
\newcommand{\changes}[1]{{\color{black}\smallskip \noindent {\bf Changes:} #1}} 

\section*{Summary of Changes}
\noindent This paper is a re-submission of a major revision decision from the second cycle of PETS '24: \textcolor{cyan}{\url{https://submit.petsymposium.org/2024.2/paper/12}}.

The following are the changes we made based on the comments from the major revision decision. 
The added changes are highlighted in the main paper using \textcolor{blue}{blue colored text}. 


\subsection*{1. Clarifying contributions} 
{\it Cleary state the contributions in comparison to related work upfront. Piecewise polynomial approximation and batch normalization are not new concepts, as pointed out with references by reviewer D. The first two points in the rebuttal, regarding positioning of Compact into existing literature and efficiency to closely related work NFGen, could be a starting point. For example, the rebuttal mentions the automatic parameter search as a distinct feature compared to related work which could be highlighted in the contributions section.}

\ans{
We clarify that, although the idea of piece-wise polynomial approximation was introduced in prior works~\cite{gilad2016cryptonets, liu2017oblivious,chabanne2017privacy,li2022mpcformer,sirnn-lib, NFGenFanCCS22}, they do not provide a mechanism to optimize 
the tradeoffs between accuracy loss and performance overhead for different complex activation functions (AFs) and DNN architectures with large number of hidden layers. 
% both negligible accuracy loss and performance overhead for deep neural networks (DNN) with many hidden layers, and complex activation functions (AFs). 
Moreover, Chabanne et al.~\cite{chabanne2017privacy}  observed that batch normalization skews the distribution of inputs received by AFs towards zero, their approach in~\cite{chabanne2017privacy} does not work for complex activation functions (line \#121-125)
}

\changes{
    In~\secref{sec:intro}, we have made changes about positioning our paper, and clarifying our contributions in light of existing literature. We positioned our paper more firmly mentioning that automatic parameter search is challenging, and we propose a new application-specific design that can find optimal parameters ensuring both negligible accuracy loss and performance overhead to solve this challenge. Furthermore, we mentioned that batch normalization (as also observed in~\cite{chabanne2017privacy}) can skew the input distribution of AFs, making polynomial approximation challenging for highly non-linear AFs.
}

\subsection*{2. Discussion of inference attacks / side-channels} 
{\it The accuracy differences due to the approximation approach and what this could reveal should be discussed. The approximation specifically provides improved accuracy for certain, e.g., more frequently appearing values compared to outliers. What possible influence can this have on inference attacks? Please include and extend the interesting discussion from the rebuttal in a revised version.}

\ans{
State-of-the-art works on secure training/inference consider membership inference (MI) attacks orthogonal to the problem~\cite{ng2023sok}. 
However, we acknowledged there could be a chance that the accuracy gap between in-distribution data and outliers may widen due to \sysname, and thus lead to an increase in MI attack success rate. However, not only ours, other existing approaches~\cite{mishra2020delphi,mohassel2017secureml} that use training or (a part of holdout data) to balance performance overhead, and accuracy loss could be susceptible to the same problem. Given that, MI attacks are more successful against outliers, we believe future work should consider, what the landscape of MI attacks will look for secure inference.}   

\changes{
    In~\secref{sec:discussion-and-futurework}, we discussed interesting avenues for future work by highlighting the need to consider adversarial attacks against ML models during secure training/inference protocols; which is largely overlooked in the existing literature. 
    Next, in the same~\secref{sec:discussion}, we gave a detailed discussion on the specific issue of MI attacks for outliers as suggested. 
    %and more in~\appref{app:membership-inference-attacks}. 
}

\subsection*{3. Extend evaluation}
{\it  Additional experiments that measure accuracy as a function of the number of activation functions and hidden layers would be helpful. Also, how does the number of layers impact the complexity of the activation function? What makes this approach more efficient than related work NFGen for models with multiple hidden layers? The rebuttal begins to address these points and we are looking forward to more details in a revised version. }

\ans{We performed an ablation study to precisely underscore what makes \sysname more efficient than NFGen~\cite{NFGenFanCCS22} by measuring the accuracy loss and performance overhead of a DNN model architecture with different numbers of hidden layers (or activation functions).
We configured \nfgen with two approximation error thresholds $\ethreshold$, one of which is borrowed from Fan et al.~\cite{NFGenFanCCS22} ($\ethreshold = 10^{-3})$, and another is a crude approximation error threshold set by us ($\ethreshold = 10^{-1}$), and compare these two with \sysname.
We found that with an increasing number of hidden layers (or activation functions), on the one hand,  
using \nfgen with a crude approximation threshold generates approximations that incur  
lower inference time; but have significant accuracy loss. On the other hand, the approximation error threshold borrowed from Fan et al.~\cite{NFGenFanCCS22} has negligible accuracy loss; but intense performance overhead. \sysname performs well in both performance overhead and accuracy loss even as the number of hidden layers increases.
}

\changes{
    In~\secref{sec:performance} with a paragraph header ``Ablation study'', we provide details of the experiment, and illustrate that our automatic parameter search coupled with incorporating batch normalization into the error function makes \sysname evidently 
    more efficient as the number of hidden layers increases for the same DNN model.
}


\subsection*{4. Expand MPC background}
{\it Provide additional information for readers not familiar with secure multi-party computation and secret sharing, so they can understand the high-level ideas and how secure computation is feasible.}

\changes{In~\secref{sec:problem-formulation} with a paragraph header ``Scenario Setup'', we gave a background on MPC protocols, as well as describe how it fits in our setup of secure inference.
}


 \subsection*{5. Expand discussion of simulated annealing}
{\it Similar to the MPC background, some more information regarding simulated annealing should be included for readers unfamiliar with that matter. Since it seems to be one of the main parts of the paper, please elaborate on how and why this technique is appropriate for this setting.}

\changes{Similarly, in~\secref{sec:time}, we gave brief details of simulated annealing (SA), and why it is used to solve the constraint optimization problem briefly in~\secref{sec:intro}, and with more details in~\secref{sec:time}. 
% We also give more details about SA in~\appref{app:minmax}.
}
\subsection*{6. Proof-read the text}
{\it Fix typos, inconsistencies, and minor comments mentioned in the reviews. Clarify sentences highlighted as unclear by the reviewers. Please make an effort to find and correct such issues in general, even if not specifically mentioned in the reviews.}

\ans{We fixed all typos and clarified all unclear sentences. We mention a few minor changes specifically suggested by the reviewers as follows.
}

% \changes{
\paragraph{Reviewer C.} 
%We move the threat model to~\appref{sec:threat-model}, and 
{ We defined $\poly_{0}$, and $\poly_{m}$ clearly in~\secref{sec:overview}. }
% We have formularized the constraint optimization problem (COP) we are solving using simulated annealing in~\secref{sec:time} (which we believe would add a bit more theoretical rigor.   

\paragraph{Reviewer B.} We added the two works~\cite{lopez2019piecewise, wang2022new} that use batch normalization for $\relu$ but fall outside the scope in~\appref{app:related-work} with a paragraph header ``Approximating AF based on batch normalization''.

\paragraph{Reviewer A.} We defined $\Time$ earlier before using it in~\secref{sec:time}.
% }
